MovieQA: Understanding Stories in Movies through Question-Answering

We introduce the MovieQA dataset which aims to evaluate automatic story comprehension from both video and text. The dataset consists of 14,944 questions about 408 movies with high semantic diversity. The questions range from simpler "Who" did "What" to "Whom", to "Why" and "How" certain events occurred. Each question comes with a set of five possible answers; a correct one and four deceiving answers provided by human annotators. Our dataset is unique in that it contains multiple sources of information -- video clips, plots, subtitles, scripts, and DVS. We analyze our data through various statistics and methods. We further extend existing QA techniques to show that question-answering with such open-ended semantics is hard. We make this data set public along with an evaluation benchmark to encourage inspiring work in this challenging domain.

==> sections/introduction1.tex <==
%!TEX root = ../cvpr2016.tex
\section{Introduction}
\label{sec:intro}

Fast progress in Deep Learning as well as the large amount of available labeled data has significantly pushed forward the performance in many visual tasks such as image tagging, object detection and segmentation, action recognition, and image/video captioning.
We are steps closer to applications such as visual solutions for the blind or cognitive robotics, which require a holistic understanding of the visual world by reasoning about all these tasks in a common framework.
However, a truly intelligent machine would ideally also infer high-level semantics behind people's (visual) actions such as motivation, intent and emotion, in order to react and, possibly, communicate appropriately.
These topics have only began to be explored in the literature~\cite{thewhy,ZhuICCV15}.

%, as well as have the ability to communicate  with the humans in natural language. %, and to react appropriately in a variety of situations.

A great way of showing one's internal understanding about the scene is to be able to answer any question about it~\cite{malinowski14nips}.
This idea gave rise to several question-answering datasets which provide a set of questions for each image along with multi-choice answers.
These datasets are either based on RGB-D images~\cite{malinowski14nips} or a large collection of static images such as Microsoft Coco~\cite{VQA,VisualMadlibs}.
The types of questions typically asked are  \emph{what} is there and \emph{where} is it, what color or shape an object has, what's its relation to other objects in the scene, and \emph{how many} objects of certain type are there in the scene.
While these questions verify the holistic nature of our vision algorithms, there is an inherent limitation to what can be asked about a static image.
High-level semantics such as motivation and intent is mostly lost and can typically only be inferred from temporal, possibly life-long visual observations.

In this paper, we argue that question-answering about movies ...
Movies provide us with snapshots from people's lives that link into stories, allowing an experienced human viewer to get a high-level understanding of the characters and their actions, the motivation behind the actions as well as the emotions they are feeling by taking them.


Our aim in this paper is to collect a large-scale question-answering dataset about movies.
Our dataset will provide a set of questions and answers with ground-truth alignment to both video and text.
This will enable the learning techniques to learn how to localize content of a particular granularity.
The challenge will then be to deal with highly varying duration of the alignment, with questions like ``What is she wearing at dinner?'' answerable with only a fraction of a second of video, while questions such as ``What is Nick and Amy's marriage like?'' requiring almost the full-length of video.
We believe that our dataset will inspire the next generation of question-answering techniques that will need to capture the true semantics of long and complex input.
We plan to create a benchmark hosted online with an active leader board.

We test a set of recently proposed QA methods on our dataset, showing...

\begin{figure*}
\centering
  \includegraphics[width=1.0\linewidth,trim=0 0 0 0,clip]{figs/MovieQA_5Q.pdf}
\vspace*{-0.6cm}
\caption{intro}
\label{fig:intro}
\end{figure*}


==> tables/qa_anstype.tex <==
%!TEX root = ../cvpr2016.tex
\begin{table}[t]
\centering
\begin{tabular}{ll}
\toprule
 Answer type              & \#QA          \\
\midrule
 Person name (who)        & 248          \\
 Reasoning (why)          & 168          \\
 Abstract (what)          & 139          \\
 Reason:action (how)      & 105          \\
 Location (where)         & 92           \\
 Action (what)            & 91           \\
 Object/Thing (what)      & 88           \\
 Person type (what)       & 87           \\
 Yes/No (is, does)        & 75           \\
 Other                    & 67           \\
 Causality (what happens) & 48           \\
 Objective (what)         & 33           \\
 Event/Time (when)        & 32           \\
 Count (how many)         & 20           \\
 Emotion (how feel)       & 19           \\
 Length (how long/far)    & 11           \\
 Age/Years (how old)      & 5            \\
 Choice (which)           & 2            \\
 ------------             & ------------ \\
 Total                    & 1330         \\
\bottomrule
\end{tabular}
\caption{Answer type stats}
\label{tab:qa_anstype}
\end{table}


==> tables/qa_firstword.tex <==
%!TEX root = ../cvpr2016.tex
\begin{table}[t]
\centering
\begin{tabular}{lrrrr}
\toprule
 First word   &   \#MA &   avg.\#w.Q &   avg.\#w.CA &   avg.\#w.WA \\
\midrule
 What         &  3323 &       9.71 &        5.69 &        4.99 \\
 Who          &  1425 &       7.42 &        2.52 &        2.18 \\
 Why          &   983 &       9.27 &        7.97 &        6.62 \\
 How          &   842 &       9.10 &        6.07 &        5.26 \\
 Where        &   537 &       8.15 &        3.57 &        3.19 \\
 When         &   122 &       9.30 &        5.32 &        4.65 \\
 Does         &    81 &      10.37 &        3.11 &        5.45 \\
 Which        &    76 &       9.17 &        2.68 &        2.40 \\
 In           &    58 &       9.16 &        3.21 &        2.87 \\
 Others       &   255 &       9.99 &        3.76 &        4.00 \\
\bottomrule
\end{tabular}
\caption{QA first word stats}
\label{tab:qa_firstword}
\end{table}


==> tables/results-simple_baseline.tex <==
%!TEX root = ../cvpr2016.tex
\begin{table}[t]
\centering
\begin{tabular}{lrrrr}
\toprule
 Method                  &   Plot &   DVS &   Subtt &   Script \\
\midrule
 TFIDF (wthr-1/2)        &  56.27 & 28.42 &   27.30 &    29.20 \\
 TFIDF (wthr-2/5)        &  53.34 & 28.63 &   26.87 &    29.20 \\
 Word2Vec (mean pooling) &  38.16 & 25.85 &   25.57 &    25.48 \\
 SkipThought             &  31.22 & 21.79 &   21.22 &    20.95 \\
 memN2N (w2v, linproj)   &   0.00 &  0.00 &    0.00 &     0.00 \\
\bottomrule
\end{tabular}
\caption{Simple baseline results}
\label{tab:results-simple_baseline}
\end{table}


==> tables/vidsrc_fullmovie.tex <==
%!TEX root = ../cvpr2016.tex
\begin{table}[t]
\centering
\begin{tabular}{rrrrr}
\toprule
   Full video &   w/ plot &   w/ subtt &   w/ trans &   w/ DVS \\
\midrule
          253 &       253 &        252 &        106 &       36 \\
\bottomrule
\end{tabular}
\caption{Video full movie counts}
\label{tab:vidsrc_fullmovie}
\end{table}


==> tables/vidsrc_stats.tex <==
%!TEX root = ../cvpr2016.tex
\begin{table}[t]
\centering
\begin{tabular}{rrlrl}
\toprule
   \#Video (aligned) &   \#QA & \#Clips   &   Clip duration (s) & Clip \#shots   \\
\midrule
                 29 &  1186 & Many! :) &              156.79 & dont know...  \\
\bottomrule
\end{tabular}
\caption{Video source stats}
\label{tab:vidsrc_stats}
\end{table}

